A Joint Learning Approach based on Self-Distillation for Keyphrase Extraction from Scientific Documents

Keyphrase extraction is the task of extracting a small set of phrases that best describe a document. Most existing benchmark datasets for the task typically have limited numbers of annotated documents, making it challenging to train increasingly complex neural networks. In contrast, digital libraries store millions of scientific articles online, covering a wide range of topics. While a significant portion of these articles contain keyphrases provided by their authors, most other articles lack such kind of annotations. Therefore, to effectively utilize these large amounts of unlabeled articles, we propose a simple and efficient joint learning approach based on the idea of self-distillation. Experimental results show that our approach consistently improves the performance of baseline models for keyphrase extraction. Furthermore, our best models outperform previous methods for the task, achieving new state-of-the-art results on two public benchmarks: Inspec and SemEval-2017.

==> Background and Related Work/base.tex <==
\subsection{Keyphrase Extraction}
\input{Background and Related Work/keyphrase_extraction}

\subsection{Self-Training}
\input{Background and Related Work/self_training}

==> Background and Related Work/keyphrase_extraction.tex <==
Keyphrase extraction is the task of automatically extracting representative phrases or concepts that concisely represent the essence of the document \cite{Hasan2014AutomaticKE,Papagiannopoulou2020ARO}. It is an important research problem, with applications in many downstream tasks such as question answering, information retrieval, document clustering and summarization \cite{d2005keyphrase,Litvak2008GraphBasedKE,Kim2010SemEval2010T5,Boudin2013KeyphraseEF}. Over the past years, researchers have proposed many methods for the task. Although details vary from method to method, many previous techniques for keyphrase extraction typically operate in two steps. In the first step, a set of \textit{candidate keyphrases} is extracted from the document using some heuristics such as POS patterns for words or n-grams \cite{Wan2008SingleDK,BennaniSmires2018SimpleUK,Sun2020SIFRankAN}. In the second step, the candidate keyphrases are predicted as keyphrases or nonkeyphrases using either supervised or unsupervised approaches. Many supervised approaches cast this task as a binary classification problem where keyphrases and non-keyphrases are used to generate positive and negative examples, respectively. Different learning algorithms have
been used to train the binary classifier, including naive Bayes \cite{medelyan-etal-2009-human,Caragea2014CitationEnhancedKE,Florescu2018LearningFR}, decision tree \cite{Turney2000LearningAF}, support vector machine \cite{Lopez2010HUMBAK}, neural network \cite{Lopez2010HUMBAK}, and ensemble-based models \cite{medelyan-etal-2009-human,Lopez2010HUMBAK,Wang2017PKUICLAS}. On the other hand, unsupervised approaches generally treat the task as a ranking problem, where the candidate phrases are ranked based on some measure of informativeness and importance. Existing unsupervised ranking approaches for keyphrase extraction include statistics-based methods \cite{el2009kp,campos2018text}, graph-based ranking algorithms \cite{Matsuo2003KeywordEF,Mihalcea2004TextRankBO,Wan2008CollabRankTA,Bougouin2013TopicRankGT,florescu-caragea-2017-positionrank,Boudin2018UnsupervisedKE}, and embedding-based ranking algorithms \cite{Papagiannopoulou2018LocalWV,BennaniSmires2018SimpleUK,Sun2020SIFRankAN}. In the presence of sufficient domain-specific labeled data, supervised keyphrase extraction methods are often reported to outperform unsupervised methods \cite{kim2013automatic,caragea-etal-2014-citation,sahrawat2020keyphrase}.

Recently, researchers have started to approach keyphrase extraction as a sequence labeling task \cite{AAAI1714628,alzaidy2019bi,sahrawat2020keyphrase}. There are several advantages to this new formulation. First, it completely avoids the candidate generation step required in previous ranking-based approaches. Instead of having to generate a long list of candidate phrases and then ranking them, the target outputs are directly predicted in one go. Second, this formulation provides a unified approach to keyphrase extraction. Under this formulation, keyphrase extraction has the same format as other popular sequence labeling tasks, such as named entity recognition and part-of-speech tagging. Therefore, it gives us the option to take advantage of existing research on sequence labeling architectures \cite{huang2015bidirectional,lample-etal-2016-neural,akbik-etal-2018-contextual}. Because of these advantages, in this work, we also adopt this formulation.

==> Background and Related Work/self_training.tex <==
Our work is inspired by the recent success of self-training \cite{paul-etal-2019-handling,yalniz2019billion,xie2020self,park2020improved}. In self-training, we first train a good teacher model on labeled data and use it to label unlabeled data, and then we finally use the original labeled data and the newly labeled data to jointly train a student model \cite{yarowsky-1995-unsupervised,riloff-wiebe-2003-learning,mcclosky-etal-2008-self}. Self-training has also been applied to several NLP tasks including parsing \cite{steedman-etal-2003-bootstrapping,mcclosky-etal-2006-effective,sagae-tsujii-2007-dependency}, part-of-speech tagging \cite{clark-etal-2003-bootstrapping}, chunking \cite{paul-etal-2019-handling} and named-entity recognition \cite{paul-etal-2019-handling}. 

Concurrent to our work, \newcite{zhu2020deep} also proposed a self-training method for utilizing unlabeled scientific articles to improve the performance of keyphrase extraction models. However, there are several key differences. First, before each training epoch, their method needs to label all the unlabeled examples and then selects the ones with high confidence scores. This would incur a lot of overhead for every single training epoch. Our approach does not suffer from this issue.

==> Tables/comparision_with_transfer_learnings.tex <==
\begin{table}[!t]
\centering
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{|l|c|c|}
\hline
\multirow{2}{*}{Approach} & \multicolumn{2}{c|}{Datasets} \\ \cline{2-3} 
 & Inspec (F1) & SemEval-2017 (F1) \\ \hline
BERT (Our implementation) & 0.596$\,\pm\,$0.003 & 0.537$\,\pm\,$0.003 \\ \hline
BERT + Simple Joint Training & 0.582$\,\pm\,$0.004 & 0.545$\,\pm\,$0.008 \\ \hline
BERT + Simple Pretraining & 0.588$\,\pm\,$0.002 & 0.548$\,\pm\,$0.004 \\ \hline
BERT + STJL & \textbf{0.601$\,\pm\,$0.004} & \textbf{0.554$\,\pm\,$0.004} \\ \hline
\end{tabular}%
}
\caption{Comparison of our joint learning approach (STJL) and other transfer learning approaches. }
\label{tab:comparison_transfer_learning}
\end{table}
